Fast Parallel Tensor Times Same Vector for Hypergraphs

Hypergraphs are a popular paradigm to represent complex real-world networks exhibiting multi-way relationships of varying sizes. Mining centrality in hypergraphs via symmetric adjacency tensors has only recently become computationally feasible for large and complex datasets. To enable scalable computation of these and related hypergraph analytics, here we focus on the Sparse Symmetric Tensor Times Same Vector (S$^3$TTVc) operation. We introduce the Compound Compressed Sparse Symmetric (CCSS) format, an extension of the compact CSS format for hypergraphs of varying hyperedge sizes and present a shared-memory parallel algorithm to compute S$^3$TTVc. We experimentally show S$^3$TTVc computation using the CCSS format achieves better performance than the naive baseline, and is subsequently more performant for hypergraph $H$-eigenvector centrality.

==> algorithms/naive_old.tex <==
\begin{algorithm}[h]
\small
    \begin{algorithmic}[1]
        \Statex \textbf{Input}: Non-uniform hypergraph stored in \cmpdformat{}, $\V{b}$
        \Statex \textbf{Output}: \sttsvc{} output, $\V{s} = \T{X}^B\V{b}^{N_k - 1}$
        \For{$l = N_k - 1, N_k - 2, \ldots ,1$}
            \ParFor{$i_l = 1, \ldots , nnz_l$}
                \If{$v_{i_l}$ owns IOU non-zeros}
                    \State \texttt{coefs} = $\sqbr*{1, b_{v_{i_l}}, \frac{b_{v_{i_l}}^2}{2!}, \ldots, \frac{b_{v_{i_l}}^{r-1}}{(r-1)!}}$
                    \State \jli{\texttt{coefs}$^\prime$ = \texttt{coefs} ? }
                    % \State \texttt{updated-coefs} = \texttt{coefs}
                    \State $u_{i_{l-1}}$ = \texttt{parent}($v_{i_l}$)
                    \For{$l^\prime = l - 1, \ldots , 1$}
                        \State \jli{$\texttt{coefs}^\prime = \texttt{coefs}^\prime \cdot b_{u_{i_{l^\prime}}}$}
                        % \State $\texttt{updated-coefs} = \texttt{updated-coefs} \cdot b_{u_{i_{l^\prime}}}$
                        \State \jli{$\texttt{coefs}^\prime = \sqbr*{0, \texttt{coefs}^\prime[0:N_k-1]}$}
                        % \State $\texttt{updated-coefs} = \sqbr*{0, \texttt{updated-coefs}[0:N_k-1]}$
                        \For{$i = 1, 2, \ldots N_k - l + 1$}
                            \State $\texttt{coefs}^\prime = \sqbr*{0, \ldots , 0, \frac{b_{u_{i_{l^\prime}}}^{i+1}}{(i+1)!} \texttt{coefs}[0:N_k-(i+1)]}$
                            % \State $\texttt{updated-coefs} = \sqbr*{0, \ldots 0, \frac{b_{u_{i_{l^\prime}}}^{i+1}}{(i+1)!} \texttt{coefs}[0:N_k-(i+1)]}$
                        \EndFor
                        \State \texttt{coefs} = \texttt{coefs}$^\prime$
                        % \State \texttt{coefs} = \texttt{updated-coefs}
                        \State $u_{i_{l^\prime-1}}$ = \texttt{parent}($u_{i_l^\prime}$)
                    \EndFor
                    \State AtomicAdd$\br*{\V{s}_{v_{i_l}}, \frac{(r-1)!l}{\alpha} \texttt{coefs}_{N_k}}$
                \EndIf
            \EndParFor
        \EndFor
    \end{algorithmic}
    \caption{\sttsvc{} using \cmpdformat{} via generating function or FFT. \jli{Add FFT in this figure as well.}}
    \label{alg:naive}
\end{algorithm}

==> algorithms/optimized_old.tex <==
\begin{algorithm}[h]
    \begin{algorithmic}[1]
        \State \textbf{Input}: Non-uniform hypergraph stored in \cmpdformat{}, $\V{b}$
        \State \textbf{Output}: \sttsvc{} output, $\V{s} = \T{X}^B\V{b}^{N_k - 1}$
        \State Allocate sub-coefficient memoization stack workspace of size $N_k \frac{(N_k - N_1)^2}{2}$
        % W \in \Rn{(N_k - N_1)\times (N_k - N_1)}$ per thread
        \ParFor{$i_1 = 1, 2, \ldots nnz_1$}
            \State Initialize $W_{ii} \leftarrow b_{v_{i_1}}, 1 \leq i \leq N_k - N_1$
            \If{subtree rooted at $v_{i_1}$ owns IOU non-zeros}
                \For{$j = 1, 2, \ldots N_k - N_1$}
                    \For{$i = 1, 2, \ldots j - 1$}
                        \State $W_{ij} \leftarrow   \frac{b_{v_{j_1}}^{j-i+1}}{(j-i+1)!}$
                    \EndFor
                \EndFor
                \State DFS($v_{i_1}$, $W$)
            \EndIf
        \EndParFor
        \Function{DFS}{$u_{i_l}$, $W$}
            \If{$v_{i_l}$ owns IOU non-zero}
                \State $u = $ left-out index at $v_{i_l}$
                \State \texttt{coefs} = $\sqbr*{1, b_{u_{i_l}}, \frac{b_{u_{i_l}}^2}{2!}, \ldots, \frac{b_{u_{i_l}}^{l-1}}{(l-1)!}}$
                \State AtomicAdd$\br*{\V{s}_{v_{i_l}}, \frac{(r-1)!l}{\alpha} \texttt{coefs}^TW_l}$
            \EndIf
            \For{$v_{i_{l+1}} \in \text{children of }u_{i_l}$}
                \If{subtree rooted at $v_{i_1}$ owns IOU non-zeros}
                    \For{$q = 1, 2, \ldots N_k - N_1$}
                        \For{$p = 1, 2, \ldots j - 1$}
                            \State $Z_{pq} \leftarrow   b_{v_{i_{l+1}}} W_{pq} + \sum\limits_{c=1}^{q-1} \frac{b_{v_{i_{l+1}}}^{c+1}}{(c+1)!} W_{p,q-c}$
                        \EndFor
                        \State $Z_{qq} \leftarrow b_{v_{i_{l+1}}} W_{qq}$
                    \EndFor
                    \State DFS($v_{i_{l+1}}$, $Z$)
                \EndIf
            \EndFor
        \EndFunction
        % \For{$l = N_k - 1, N_k - 2, \ldots 1$}
        %     \ParFor{$i_l = 1, \ldots nnz_l$}
        %         \If{$v_{i_l}$ owns IOU non-zero}
        %             \State \texttt{coefs} = $\sqbr*{1, b_{v_{i_l}}, \frac{b_{v_{i_l}}^2}{2!}, \ldots, \frac{b_{v_{i_l}}^{r-1}}{(r-1)!}}$
        %             \State \texttt{updated-coefs} = \texttt{coefs}
        %             \State $u_{i_{l-1}}$ = \texttt{parent}($v_{i_l}$)
        %             \For{$l^\prime = l - 1, \ldots 1$}
        %                 \State $\texttt{updated-coefs} = \texttt{updated-coefs} \cdot b_{u_{i_{l^\prime}}}$
        %                 \State $\texttt{updated-coefs} = \sqbr*{0, \texttt{updated-coefs}[0:N_k-1]}$
        %                 \For{$i = 1, 2, \ldots N_k - l + 1$}
        %                     \State $\texttt{updated-coefs} = \sqbr*{0, \ldots 0, \frac{b_{u_{i_{l^\prime}}}^{i+1}}{(i+1)!} \texttt{coefs}[0:N_k-(i+1)]}$
        %                 \EndFor
        %                 \State \texttt{coefs} = \texttt{updated-coefs}
        %             \EndFor
        %             \State AtomicAdd$\br*{\V{s}_{v_{i_l}}, \frac{(r-1)!l}{\alpha} \texttt{coefs}_{N_k}}$
        %         \EndIf
        %     \EndParFor
        % \EndFor
    \end{algorithmic}
    \caption{Memoized \sttsvc{} using \cmpdformat{} and generating function.}
    \label{alg:optimized}
\end{algorithm}

==> algorithms/without-css_old.tex <==
\begin{algorithm}
\scriptsize
    \begin{algorithmic}[1]
        \State \textbf{Input}: rank $r$ hypergraph $(V,E)$, vector $\V{b}$
        \State \textbf{Output}: \sttsvc{} output, $\V{s} = \T{X}^B\V{b}^{N_k - 1}$
        \For{$v\in V$}

                    \State $c \gets 0$
                    \For{$e\in E(v)$}
                        \State $c\pluseq \displaystyle\frac{|e|}{\alpha} (r-1)! \left(\exp({\Vc{b}_vt}) \prod_{ \substack{ u \in e \\ u \neq v}}(\exp({\Vc{b}_ut}) -1)\right)[t^{r-1}]$
                    \EndFor
        \State $\V{s}_v \gets c$
        \EndFor
        \State \bf{return} $\V{s}$
    \end{algorithmic}
    \caption{AAY algorithm for implicit TTSV1 using Banerjee adjacency tensor. \jli{Exact the same with the published paper?}
    \sjy{alpha isn't defined and do we want to say a rank $N_k$ hypergraph or rank $r$?}}
    \label{alg:without-css}
\end{algorithm}

==> summary-of-changes.tex <==
% LaTeX rebuttal letter example. 
% 
% Copyright 2019 Friedemann Zenke, fzenke.net
%
% Based on examples by Dirk Eddelbuettel, Fran and others from 
% https://tex.stackexchange.com/questions/2317/latex-style-or-macro-for-detailed-response-to-referee-report
% 
% Licensed under cc by-sa 3.0 with attribution required.
% See https://creativecommons.org/licenses/by-sa/3.0/
% and https://stackoverflow.blog/2009/06/25/attribution-required/

% \documentclass[11pt]{article}
% \usepackage[utf8]{inputenc}
% \usepackage{lipsum}
% \usepackage{fullpage}

% \usepackage{xr}
% \makeatletter
% \newcommand*{\addFileDependency}[1]{% argument=file name and extension
%   \typeout{(#1)}
%   \@addtofilelist{#1}
%   \IfFileExists{#1}{}{\typeout{No file #1.}}
% }
% \makeatother
% \newcommand*{\myexternaldocument}[1]{%
%     \externaldocument{#1}%
%     \addFileDependency{#1.tex}%
%     \addFileDependency{#1.aux}%
% }
% \myexternaldocument{tex/background}
% \listfiles

% \usepackage{cleveref}
% \Crefname{equation}{Eq.}{Eqs.}
% \Crefname{figure}{Fig.}{Figs.}
% \Crefname{tabular}{Tab.}{Tabs.}
% \Crefname{section}{Sec.}{Secs.}
% \crefname{thm}{theorem}{theorems}
% \Crefname{thm}{Theorem}{Theorems}
% \crefname{prop}{property}{properties}
% \Crefname{prop}{Property}{Properties}

% % import Eq and Section references from the main manuscript where needed

% % package needed for optional arguments
% \usepackage{xifthen}



% \begin{document}
\newpage
\section*{Response to the reviewers}
We thank the reviewers for their critical assessment of our work. 
In the following, we have addressed the concerns point by point and revised the paper accordingly.

\reviewersection
\textbf{Reasons to accept} This reviewer has zero background in the topic of this paper but found the paper refreshingly readable. The examples helped illuminate the core data structure and the discussion motivated well the transition to a top-down traversal and to the introduction of memoization. The experiments were also well-described and show clear improvements over the state of the art. And this reviewer particularly appreciated the succinct but useful performance analysis on understanding which CCSS methods were most performant for which type of hypergraph dataset.

\textbf{Areas of improvement} I have no significant areas of improvement.

\begin{point}
    What this reviewer cannot ascertain is the significance of this operation. This reviewer cannot offer an expert opinion on this. It is not clear to this reviewer that hypergraph centrality is an important kernel in real-world scenarios.
\end{point}
\jli{try to find more application scenarios.}

\begin{point}
I might consider a paper title that better expresses what a user can do with an efficient implementation of \sttsvc{}. The title, as it is, is pretty specialized to only experts who know this particular operation, but the authors surely want this data structure and computational method to be made aware to a broader audience.
\end{point}
\begin{reply}
We thank the reviewer for the thoughtful comment. \shrshi{How about "Parallel tensor eigendecomposition for hypergraph centrality using compound sparse storage"} \jli{Our work is not very specific, try to get more application to support. And one this reviewer posted this Q, we don't want to make a big change on the title.}
\end{reply}

\shortpoint{Cites are not words. You must be able to delete the cite and the sentence make sense. (e.g., "In [13]", "see [22]", "from [12]")}
\shortreply{Addressed.}

\shortpoint{The text uses many hyphens (-) in body text as dashes that should, typographically, be en-dashes (--) or em-dashes (---).}
\shortreply{Addressed.}

\shortpoint{IV.A., first paragraph. Double use of "algorithm Algorithm", and "in efficient" -> "inefficient".}
\shortreply{Fixed.}

\shortpoint{Figure 6 is a good visualization and supports the scalability argument well.}

\begin{point}
    \textit{(Rebuttal)}
    
    Is there any significant memory footprint impact from using memoization?
\end{point}
\begin{reply}
    The memory footprint due to the \cmpdformat{} is at least $2^{N_k}$, where $N_k$ is the largest hyperedge cardinality. The memoization overhead of storing the $\M{W}$ matrix is of the order $N_k^2$. The memoization overhead is not significant relative to the size of the \cmpdformat{} required to store the non-uniform hypergraph.\jli{We will add an extra paragraph to explain the memory footprint of CCSS-MEMO.} \jli{make the comparison more clear.}
\end{reply}



% Begin a new reviewer section
\reviewersection
\textbf{Reasons to accept}
    This paper addresses an important and interesting problem: optimizing the tensor-times same vector operation for tensors relevant to non-uniform hypergraphs. This is a key kernel in hypergraph centrality algorithms.
    The authors obtain excellent speed-up over the previous state-of-the-art algorithm for the kernel under consideration.
    The paper was generally well-organized and well-written.

\textbf{Areas of improvement}
Extending the algorithm for the CSS format from \cite{Shivakumar2021EfficientTensors} and \cite{Shivakumar2023SparseDecomposition} (cited in paper) to Algorithm 4 for the CCSS format in the present work, although important in terms of applications, may be of incremental novelty/effort. 

\begin{point}
Please highlight the difficulties in extending the algorithms in \cite{Shivakumar2021EfficientTensors} and \cite{Shivakumar2023SparseDecomposition} (cited in paper) to Algorithm 4 in the present work.
\end{point}
\begin{reply}
Shivakumar et al. \cite{Shivakumar2021EfficientTensors,Shivakumar2023SparseDecomposition} outlines an efficient parallel algorithm for uniform hypergraph clustering using the symmetric Tucker decomposition of the adjacency tensor stored in the \format{} format. As non-uniform hypergraphs are comprised of component uniform hypergraphs, the challenge posed in directly applying the tensor decomposition idea to non-uniform hypergraphs is the aggregation of the factor matrices obtained from the decomposition of each component symmetric adjacency tensor. Since the factor matrix is a low-rank node-embedding of the component uniform hypergraph, the update step in the iterative decomposition algorithm is not trivial, and its dependence on the component hypergraph order requires further study. An alternative representation of the non-uniform hypergraph is the \blowup{} tensor. The \format{} format can be used to store the explicitly constructed \blowup{} tensor. However, due to the combinatorial expansion of the hyperedges in the \blowup{} tensor construction, the size of the \format{} will be prohibitively large. The \cmpdformat{}, which stores only the hyperedges of the non-uniform hypergraph, facilitates the implicit construction and decomposition of the \blowup{} tensor thereby providing insights into the structure of non-uniform hypergraphs. \jli{We will add more explanations to XX.} \jli{Make this paragraph more compact and to the point.} 
\end{reply}

\shortpoint{In \Cref{eq:ttsv1}, change the subscripts $r$ to $N$.}
\shortreply{Fixed.}

\shortpoint{Consider using a different letter/notation for hypergraphs: H=(V,E)
, and weighted hypergraphs H=(V,E,w)
, to avoid confusion.}

\shortpoint{I believe that you need to assume that the hypergraph is connected to guarantee the existence/uniqueness of the strictly positive H-(eigenvalue, eigenvector) pair; please note this in the paper.}

\shortpoint{In Figs. 1 and 2, color-code all of the $v_i$ values for consistency.}
\shortreply{Fixed.}

\shortpoint{In Section III, 5th line: change 'naturally' to 'natural'.}
\shortreply{Fixed.}

\shortpoint{Change 'in efficient' to 'inefficient' in 5th line under Algorithm 3.}
\shortreply{Fixed.}

\begin{point}
    \textit{(Rebuttal)}
    
    Does the extension of the algorithms from \cite{Shivakumar2021EfficientTensors} and \cite{Shivakumar2023SparseDecomposition} (cited in paper) to Algorithm 4 in the present work require significant effort?
\end{point}
\begin{reply}
    Shivakumar et al. \cite{Shivakumar2021EfficientTensors,Shivakumar2023SparseDecomposition} outlines an efficient parallel algorithm for uniform hypergraph clustering using the symmetric Tucker decomposition of the adjacency tensor stored in the \format{} format. As non-uniform hypergraphs are comprised of component uniform hypergraphs, the challenge posed in directly applying the tensor decomposition idea to non-uniform hypergraphs is the aggregation of the factor matrices obtained from the decomposition of each component symmetric adjacency tensor. Since the factor matrix is a low-rank node-embedding of the component uniform hypergraph, the update step in the iterative decomposition algorithm is not trivial, and its dependence on the component hypergraph order requires further study. An alternative representation of the non-uniform hypergraph is the \blowup{} tensor. The \format{} format can be used to store the explicitly constructed \blowup{} tensor. However, due to the combinatorial expansion of the hyperedges in the \blowup{} tensor construction, the size of the \format{} will be prohibitively large. The \cmpdformat{}, which stores only the hyperedges of the non-uniform hypergraph, facilitates the implicit construction and decomposition of the \blowup{} tensor thereby providing insights into the structure of non-uniform hypergraphs. \jli{We only needs to keep P2.8 not P2.1.}
\end{reply}

\reviewersection
\textbf{Reasons to accept}

Novel data structure and algorithm design

Testing and analysis of results

Comprehensive solution with application

\begin{point}
Plots can be improved a bit. In particular, the text where Figure 4 is referred to mentions a 50x speedup for CCSS-MEMO over CCSS-DIRECT. The figure does not indicate which instance attains this speedup. Some labels may be added to the bars in Figure 4 to provide more clarity.
\end{point}
\jli{What is the answer for this Q?}

\begin{point}
    The plot on scalability shows information for up to 64 threads, whereas Figure 4 is apparently using 128 threads. Why this discrepancy? As it appears from Figure 6 that CCSS-Direct has better scalability than CCSS-MEMO, the absence of the data point corresponding to 128 threads is all the more interesting. 
\end{point}
\begin{reply}
    \shrshi{We had done this so that \Cref{fig:s3ttvc-runtime} shows the overall performance of the three approaches and \Cref{fig:s3ttvc-scalability} shows the scalability of the three algorithms. \jli{We tried not to duplicate the same numbers in different figures to show more results.} }
\end{reply}

\begin{point}
    \textit{(Rebuttal)}
    
    The authors may consider addressing the scalability issue of the proposed approach. This is one aspect which is not convincingly done/reported in the paper.
    The authors may justify the lack of good scalability for the proposed algorithm wrt its usability in multi-threaded environments. There appears to be some questions around the design of the algorithm/data structure/ program that may make the approach hit a wall due to poor scalability. 
\end{point}
\jli{An important Q to answer}

\begin{point}
    \textit{(Rebuttal)}

    I do not see great value add from Table 2.
\end{point}

\reviewersection
\textbf{Reasons to accept} This paper tackles a fairly complex algorithmic task of efficiently computing a key kernel in processing hypergraph adjacency tensors. The real-world applications of this kernel and hypergraph processing are obvious and well articulated. The paper clearly describes the state-of-art, identifies the areas of improvement, and proposes improved algorithms with well-reasoned arguments. While the discussion is quite dense, the ideas underpinning the improvements, namely an efficient storage format, and exploiting memoization while using this format, are fully plausible. The results are presented for a comprehensive set of experiments that appear to back up most, if not all, of the expected benefits.

\textbf{Areas of improvement} The clarity of the overall discussion can (and should) be significantly improved. The arguments made by the authors are sound, but the exposition is dense and very confusing at many places, leading me to think that the paper is rather hastily written. The topic deserves a much more clear presentation. 

\begin{point}
    The two main algorithmic contributions, the CCSS format, and the memoization algorithm (Algo 4) deserve more clarity. For e.g., the use of the example is Figs. 1 and 2 is very appropriate, but the accompanying text is confusing. The last sentence above sec. III-A mentions "edge {1, 4, 5}" but I do not see any such edge (a polygon encircling 1, 4, and 5 in Fig. 1). 
\end{point}

\begin{point}
    \textit{(Rebuttal)}
    
    When the memoization algorithm is presented, the authors could have continued to illustrate with the example in Figs. 1 and 2. For e.g., illustrating the memoization space matrix W for a couple of vertices would have greatly improved clarity. Without this its very difficult what exact "memoization" is being exploited. In fact the section III-B appears too concise, and doesn't do justice for the intricacies of the algorithm. It is mentioned that a "separate memoization space, W" is used for each tree. Does this mean a separate W is allocated for each of the vertices v? Line-1 of Algo 4 says $W_i$, but its not clear what the subscript "i" refers to.
\end{point}
\begin{reply}
    The memoization workspace is allocated per processor, which stores the $\M{W}$ matrix of convolution operations. Moreover, note that the off-diagonals of $\M{W}$ are constant, which is another optimization implemented to bring down memory costs. \jli{Combine this Q with P1.7 into a big memoization Q, but still separate as two sub-Qs if they are different.}
\end{reply}

\begin{point}
    \textit{(Rebuttal)}
    
    The experiments are comprehensive, but the authors wade into murky waters making comparisons to, and claiming improvements over, the SOTA algorithm from ref [13]. Its always difficult getting the best possible implementation of someone else's algorithm, and the authors acknowledge that in footnote \#3. But regardless, the improvements of their CCSS-FFT and CCSS-MEMO over CCSS-DIRECT are obvious, and these constitute sufficient novelty. My suggestion would be to severely temper their conclusions in terms of improvements w.r.t. the algorithm of [13], and rather highlight the improvements due to adopting the CCSS format, and the FFT and MEMO variants relative to the DIRECT algorithms.
\end{point}

\begin{point}
    \textit{(Rebuttal)}
    
    There is no discussion on memory footprint. The improvements surely comes at the cost of higher memory requirements; both the FFT and memoization seem to need it. Some discussion on this cost and the tradeoff w.r.t. computational time would make the discussion complete.
\end{point}

\begin{point}
    The paper has many typos, incomplete or mangled sentences, and certain abbreviations are introduced without being defined (e.g. CCSS-FFT on page 1, S3TTMc on page 3).
\end{point}

\reviewersection
\textbf{Reasons to accept} The authors tackle a complex algorithm space with non-uniform hypergraphs and develop a shared memory algorithm for improving the CSS approach used for uniform hypergraphs.

Writing and presentation are good in general, with a few minor grammar and spacing issues.

The authors present a new compound version of the Compressed Sparse Symmetric format for non-uniform hypergraphs as well as a parallel implementation of \sttsmc. The work seems to be novel and the paper is well-written. Results show noticeable speed-up, although it is somewhat unclear if there are related approaches that can be compared as baselines.

\begin{point}
    Is there a possible baseline that is not CCSS derived that you can refer to or compare against in more detail? It is understandable that this is a somewhat niche algorithm but listing speedup compared to the newly developed CCSS seems somewhat misleading and may lead readers to wonder how this work fits in with other state-of-the-art approaches. Table 2 sort of addresses this but it's not clear this Python algorithm is CSS-derived or even related without a more detailed evaluation of related work.
\end{point}

\begin{point}
    It would be nice to see a Figure like Figure 1 that demonstrates the key differences between CSS and CCSS for a small hyper graph.
\end{point}
\begin{reply}
    \shrshi{We need to clarify that the \format{} format is for uniform hypergraphs and \cmpdformat{} is for non-uniform hypergraphs?}
\end{reply}

\begin{point}
    \textit{(Rebuttal)}
    
    You mention the limitations of CSS as a reason why CCSS is needed as an extension for non-uniform hypergraphs. Do you have a sense as to how much faster CCSS would be than CSS if someone put in the engineering effort to implement a CSS approach, as stated in Section 3?
\end{point}
\begin{reply}
    The symmetric \blowup{} tensor used to represent adjacency information in non-uniform hypergraphs is constructed by combinatorially expanding the lower-cardinality hyperedges to that of the rank of the hypergraph. Note that explicitly constructing the \blowup{} tensor and storing it in the \format{} format will be compute- and memory-intensive owing to the number of IOU non-zeros that need to be generated and stored. An alternative choice is to instead adopt the implicit construction approach and store the hypergraph using a \format{} format for each component symmetric adjacency tensor. Not only is this approach suboptimal in terms of memory requirement compared to \cmpdformat{}, we also pay the penalty of greater computation cost since we lose out memoizing intermediate $\bar{E}_N$ across IOU non-zeros i.e. hyperedges. \jli{This Q can be merged as well, with P2.8.}
\end{reply}

==> tex/compound-css_old.tex <==
\section{Compound CSS Structure}
The \format{} structure \cite{Shivakumar2021EfficientTensors,Shivakumar2023SparseDecomposition} is a compact storage format that enables efficient \sttsmc{} computation for sparse symmetric adjacency tensors arising from uniform hypergraphs. In this paper, we present an extension of \format{}, called \cmpdformatfull{} (\cmpdformat{}) which facilitates fast \sttsvc{} computation on the \blowup{} tensor representing non-uniform hypergraphs.
% to store non-uniform hypergraphs, and adapt it for \sttsvc{} operation on the symmetric Banerjee tensor representation of non-uniform hypergraphs. 

We first summarize the \format{} format. For a symmetric tensor $\T{X} \in \Rn{n \times n \times \ldots n}$ of order $N$, \format{} is a forest with $N-1$ levels constructed from IOU \sga{First time using this here -- is it necessary to define it as ``index-ordered unique"?} non-zeros, $unz(\T{X})$. A key advantage of using the \format{} format is its computation-aware nature - by storing all ordered subsequences of IOU non-zeros, intermediate results in the \sttsmc{} computation can be easily memoized with minimal additional index information. The \format{} format admits the following property - any path $\mathcal{P}_{\V{i}_l}$ is a $l$-length subsequence of the index tuple $\V{i}$ of some IOU non-zero, i.e. each IOU non-zero corresponds to multiple paths $\mathcal{P}_{\V{i}_l}$ to levels $l = 1, 2, \ldots N-1$. For a single IOU non-zero, the number of nodes at level $l$ is $\binom{N}{l}$ for \format{}.
% We need to save both pointers and indices for every level, which doubles the storage of \format.
The affiliated leaf level indices and non-zero values are stored in each of the $N$ nodes at level $(N-1)$ generated by this non-zero.

The \cmpdformat{} extends the \format{} to non-uniform hypergraphs by storing all of the $k$ component uniform hypergraphs in the same structure. \cmpdformat{} is constructed as a forest with $N_k - 1$ levels, with the values of IOU non-zeros of $\T{X}_l$ stored at level $N_l - 1$ for $1 \leq l \leq k$. A path $\mathcal{P}_{\V{i}_l}$ from level 1 to level $l$ corresponds to an ordered subsequence of size $l$ contained in at least one IOU non-zero across all component adjacency tensors $\T{X}_l, 1\leq l \leq k$. Such a construction enables reuse of paths across tensors without having to construct separate \format{} formats for each tensor.
In the example shown in \Cref{fig:ccss}, the \cmpdformat{} is constructed from a 8-node weighted non-uniform hypergraph with the 6 IOU non-zeros shown in \Cref{tab:example}. It consists of three component uniform hypergraphs, giving rise to adjacency tensors $\T{X}_1, \T{X}_2$, and $\T{X}_3$ of order 2, 3, and 4 respectively. The IOU non-zeros are stored at levels 1, 2, and 3 in the \cmpdformat{} format, as opposed to only level 3 in the \format{} format. The reuse of paths across non-zeros is also evident from this example - path (1, 4) is shared between non-zeros (1, 3, 4, 6; $v_2$) and (1, 4, 6; $v_5$).
An IOU non-zero in $\T{X}_l$ with index set $\V{i}$ is stored at node $i_{N_l - 1}$ with the left-out index $i_{N_l} = \V{i} \setminus \mathcal{P}_{i_{N_l - 1}}$ for all $i_{N_l} \in \V{i}$. In the example, the non-zero $v_5$ is stored 3 times in the \cmpdformat{} at level 2. One of those instances is at node-4 in path $\mathcal{P}_4 = (1, 4)$, which stores the auxiliary information $[6; v_5]$. 

% Let us consider a non-uniform hypergraph as a collection of uniform hypergraphs; i.e., a sequence of symmetric adjacency tensors of increasing tensor orders. \cmpdformat{} constructs \format{} for the adjacency tensor with the largest tensor order, and uses the subsequence property described above to append the IOU non-zeros in tensors of smaller orders at lower levels of the \format{} structure.
% If the non-uniform hypergraph is composed of $N_1-, N_2-, \ldots N_k-$uniform hypergraphs generating symmetric adjacency tensors $\T{X}_1, \T{X}_2, \ldots \T{X}_k$, $N_1 < N_2 < \ldots < N_k$ then the \cmpdformat{} constructs \format{} with $N_k - 1$ levels, and inserts the IOU non-zeros of adjacency tensor $\T{X}_l$ at level $N_l - 1$, thus enabling reuse of paths across tensors without having to construct separate \format{} formats for each tensor. The sequence of three sparse symmetric tensors in \Cref{tab:example} consisting of 6 IOU non-zeros in total can be represented by the \cmpdformat{} format shown in \Cref{fig:ccss}. The non-zeros are stored at levels 1, 2, and 3 in the \cmpdformat{} format, as opposed to only level 3 in the \format{} format. 
\input{tables/hypergraph}
\input{figs/ccss}

\subsection{Space complexity}
The total number of nodes in the \cmpdformat{} depends not only on the distribution of the IOU non-zeros, but also on the distribution of the tensor orders over all component symmetric adjacency tensors. A single IOU non-zero in $\T{X}_l$ contributes $\binom{N_l}{l}$ nodes to all levels $1 \leq l \leq N_l - 1$, and $2^{N_l} - 1$ nodes in total. However, due to overlap of nodes across IOU non-zeros within a component adjacency tensor and across adjacency tensors, the number of nodes in \cmpdformat{} is much smaller than $\sum_{l=1}^k 2^{N_l} unnz(\T{X}_l)$. 

In the next section, we outline how \cmpdformat{} can be used to compute \sttsvc{} on the \blowup{} tensor while storing only the IOU non-zeros; i.e., without the combinatorial blowup.

==> tex/preliminaries_old.tex <==
\section{Preliminaries} \label{sec:preliminaries}
Following Kolda and Bader~\cite{Kolda2009TensorApplications}, we denote vectors using bold lowercase letter (e.g., \V{i}, \V{j}), matrices using bold uppercase letters (e.g., $\M{U}$), and tensors using bold calligraphic letters (e.g., $\T{X}$).

Formally, a hypergraph is a pair $H=(V, E)$, where $V$ is the set of vertices, and $H$ is the set of hyperedges on those vertices; that is, $E$ is some subset of the power set of $V$. We say $H$ is uniform if all hyperedges have the same size; otherwise, it is nonuniform. The rank of $H$ is the size of the largest hyperedge. 

An order-$N$ symmetric tensor $\T{X}$ has $N$ modes or dimensions, and is a general tensor with the special property that non-zero values, $\T{X}_{(i_1, i_2, \ldots i_N)}$ remains unchanged under any permutation of its indices. We observe sparse symmetric tensors in several contexts, one of which are those originating from hypergraphs. A $N$-uniform hypergraph on $n$ vertices, where every hyperedge spanning multiple vertices has the same cardinality $N$, can be represented as an order-$N$ symmetric adjacency tensor $\T{X} \in \Rn{n \times n \times \ldots n}$. That is, for every hyperedge $e = \{v_{i_1}, v_{i_2}, \ldots, v_{i_N} \} \in E$ with weight $w(e)$, $\T{X}_{\sigma(\V{i})} = w(e)$, where $\sigma(\V{i})$ denotes any of the $N!$ permutations of the index tuple $\V{i} = (i_1, \ldots, i_N)$.
We refer to a non-zero $\T{X}_{\V{i}} \in unz(\T{X})$ as an \emph{index-ordered unique (IOU) non-zero} if the index set $\V{i}$ is ordered ($i_1 < i_2 < \ldots < i_N)$.\sjy{Shouldn't these be $\leq$?} Thus, the hyperedges of the uniform hypergraph for the set of IOU non-zeros $\br*{unz(\T{X})}$ of $\T{X}$. \sjy{This sentence doesn't going anywhere -- it looks like the first clause for something.}

In order to expand our exposition to non-uniform hypergraphs, consider a $n$-node rank-$N_k$ non-uniform hypergraph composed of $N_1-, N_2-, \ldots N_k-$uniform hypergraphs, $N_1 < N_2 < \ldots < N_k$. Each $N_l-$uniform hypergraph induces an order-$N_l$ sparse symmetric adjacency tensor $\T{X}_l \in \Rn{n \times n \times \ldots n}$ with the set of IOU non-zeros given by $unz(\T{X}_l) = \cbr*{e \in E(H) : e = (v_{i_1}, v_{i_2}, \ldots v_{i_{N_l}}), v_{i_p} < v_{i_q} \forall p < q}$. \sjy{Is there a reason to consider the hypergraph partitioned by edge sizes? It seems like it would be shorter/cleaner to just introduce the Banerjee tensor directly from the hypergraph} A technique to unify this $N_k$-tensor representation into a single tensor is the symmetric \blowup{} tensor representation, $\T{X}^B$ \cite{Banerjee2017SpectraHypergraphs}. 
% We denote by $\T{X}^B$ the symmetric \blowup{} tensor representation \cite{Banerjee2017SpectraHypergraphs} of a non-uniform hypergraph.
$\T{X}^B$ is an order-$N_k$ tensor constructed from hyperedge blowups - for IOU non-zero $\T{X}_{l_{\V{e}}} \in unz(\T{X}_l)$ with index set $\V{e}$, blowups $\beta$ and unordered blowups $\kappa$ are defined as
\begin{align*}
    \beta(\V{e}) &= \cbr*{i_1, i_2, \ldots i_{N_k} : \text{foreach } v \in \V{e}, \exists j \ni i_j = v}\\
    \kappa(\V{e}) &= \cbr*{x : x \text{ is size } N_k \text{ multiset with support } \V{e}}
\end{align*}
$\T{X}^B$ inserts non-zeros at positions corresponding to the blowups of hyperedges, with value proportional to the size of that hyperedge's blowup set, $|\beta|$ \cite{Aksoy2023ScalableHypergraphs}. 
% Thus, $\T{X}^B$ is order-$N_k$ symmetric tensor constructed from the edges in the hypergraph such that for each edge $e_i = \br*{v_{j_1}, v_{j_2}, \ldots, v_{j_{N_l}}}, 1\leq l \leq k$, 
% $$\T{X}^B_{a_1, a_2, \ldots a_{N_k}} = \frac{N_l}{\alpha},\, \text{where }\alpha = \sum_{\substack{b_1, \ldots b_{N_l} \geq 1\\\sum b_p = N_k}} \frac{N_k!}{b_1!b_2!\ldots b_{N_l}!}$$
% and $(a_1, a_2, \ldots a_{N_k})$ are chosen in all possible ways from $\{j_1, j_2, \ldots j_{N_l}\}$ with each element from the set appearing at least once.
\sga{There is a more compact definition of this, either using/defining ``blowups" or by using stirling numbers if you want to avoid introducing blowups. Lastly, there are three authors on the ``Banerjee" paper so I wonder if just calling it the Banerjee tensor is best?}
\shrshi{the definition using blowups has been used instead}

Similar to the \sttsmc{} operation on sparse symmetric tensors \cite{Shivakumar2021EfficientTensors}, we define the \underline{S}parse \underline{S}ymmetric \underline{T}ensor \underline{T}imes \underline{S}ame \underline{V}ector (\sttsvc{}) operation on the \blowup{} tensor. \sjy{This is not a different operation, and it doesn't really matter thant it is sparse}
% Given an order-$N$ symmetric tensor $\T{X} \in \Rn{n \times n \times \ldots n}$ and vector $\V{b} \in \Rn{n}$, we have
\begin{equation}\label{eq:s3ttvc}
    \V{s} = \T{X}\V{b}^{N-1} = \T{X} \times_{-1} \sqbr*{\V{b}}
    = \T{X} \times_2 \V{b} \times_3 \V{b} \ldots \times_N \V{b}
\end{equation}
\sttsvc{}, given by \Cref{eq:s3ttvc}, is represented by a sequence of tensor times vector products (TTV)~\cite{Kaya2018ParallelTrees} on all but one mode of the symmetric tensor $\T{X}$. TTV of an order-$N$ symmetric tensor $\T{X} \in \Rn{n \times n \ldots n}$ with vector $\V{b} \in \Rn{n}$ along mode $m$, denoted by $\T{Z} = \T{X} \times_m \V{b}^T$, is defined as 
$\T{Z}_{i_1 \ldots i_{m-1} i_{m+1} \ldots i_N} = \sum_{i_m = 1}^n \T{X}_{i_1 \ldots i_{m-1} i_m i_{m+1} \ldots i_N} \V{b}_{i_m}$. Using this definition in \Cref{eq:s3ttvc}, we get 
\begin{equation}\label{eq:ttsv1}
s_{i_1} = \left[\T{X}\Vc{b}^{N-1}\right]_{i_1} = \sum_{i_2=1}^n\cdots\sum_{i_r=1}^n\T{X}_{i_1,\dots,i_r}\prod_{k=2}^N\Vc{b}_{i_k},
\end{equation}


\shrshi{Replace TTSV1 with \sttsvc{}?}
This work focuses on speeding up and parallelizing the tensor times same vector in all modes but one (TTSV1 \jli{Use a different name?}) for the \blowup{} tensor. Formally, given an order $r$ tensor $\T{X}$ and a vector $\Vc{b}\in\R^n,$ 
$\T{X}\Vc{b}^{r-1}\in\R^n$ is the TTSV1 operation given by \Cref{eq:ttsv1}.
% \begin{align}\label{eq:ttsv1}
% \left[\T{X}\Vc{b}^{r-1}\right]_{i_1} &= \sum_{i_2=1}^n\cdots\sum_{i_r=1}^n\T{X}_{i_1,\dots,i_r}\prod_{k=2}^r\Vc{b}_{i_k},
% \end{align}
ƒIn  \cite{Aksoy2023ScalableHypergraphs}, Aksoy, Amburg and Young proposed the implicit AAY algorithm to evaluate TTSV1 for the \blowup{} tensor that relies on generating functions.
The fundamental observation which drives their algorithm is that, in the \blowup{} tensor, all entries corresponding to a single edge have the same coefficient.  Thus, by using generating functions, the contributions to an entry of TTSV1 from  all entries in the \blowup{} tensor corresponding to an edge may calculated simultaneously. More concretely, the entries of the \blowup{} tensor corresponding to a particular vertex $v$ in the TTSV1 vector and edge $e$ in the hypergraph can be thought of as particular subclass of all words formed from the vertices in $e$. Apply standard generating function techniques, see \cite{} \shrshi{missing citation?}, this results in the algorithm shown in ~\Cref{alg:without-css}.
\input{algorithms/without-css}
Here, $[t^{r-1}]$ represents the coefficient of the $r-1$ degree term in the power series. The coefficient may be obtained by performing the polynomial multiplication using direct convolution, a subset expansion approach, \shrshi{isn't the direct convolution same as the subset expansion approach?} or an FFT convolution approach~\cite{Aksoy2023ScalableHypergraphs} -- and then taking the corresponding coefficient from the resulting polynomial.

While the aggregation over vertex-edge pairs given by the approach of Aksoy, Amburg, and Young results in significant computational speedups, the lack of structure imposed on the computation  results in frequent repetition of generating function convolutions. For example, in the AAY approach the product $(\exp(\Vc{b}_vt)- 1)(\exp(\Vc{b}_ut) -1)$ is computed $|e|-2$ times for every edge containing both $v$ and $u$.

% EXPLAIN the advantage of CSS vs. this approach.
